Symbolic Abstract Heaps for Polymorphic Information-flow Guard Inference (Extended Version)

In the realm of sound object-oriented program analyses for information-flow control, very few approaches adopt flow-sensitive abstractions of the heap that enable a precise modeling of implicit flows. To tackle this challenge, we advance a new symbolic abstraction approach for modeling the heap in Java-like programs. We use a store-less representation that is parameterized with a family of relations among references to offer various levels of precision based on user preferences. This enables us to automatically infer polymorphic information-flow guards for methods via a co-reachability analysis of a symbolic finite-state system. We instantiate the heap abstraction with three different families of relations. We prove the soundness of our approach and compare the precision and scalability obtained with each instantiated heap domain by using the IFSpec benchmarks and real-life applications.

==> fig/scfg-gen-setup.tex <==
% -*- coding: utf-8; mode: latex -*-
\tikzset{%
  every node/.style={align = center, inner sep = 1.2pt},
  every path/.style={line width=.5pt},
  align = center,
  anchor = center,
}%
\tikzstyle{location} =%
[ draw
, rectangle
% , font=\smaller
]%
\tikzstyle{label} = [font=, inner sep = 0pt, outer sep = 0pt]%
\tikzstyle{label'} = [label, outer sep = 1pt]%
\tikzstyle{label''} = [label, inner sep = 1pt, outer sep = 2pt, font=, draw = analysis, dashed]%
\colorlet{basic}{black}%
\colorlet{nominal}{blue!50!black}%
\colorlet{analysis}{green!20!black}%
\tikzstyle{basic-arrow} = [->, basic]%
\tikzstyle{nominal-arrow} = [->, nominal]%
\tikzstyle{analysis-arrow} = [->, analysis% , decorate, decoration = {%
  % snake, amplitude = .2mm, segment length = 1mm, post length = 1.4mm}
]%
\colorlet{semloc}{red!60!black}%
\tikzstyle{semloc-label} = [semloc, font=]%
%
\tikzstyle{overlay-arrow} = [%
, thick
, >=stealth
, dashed
, white!70!black
% , line width = 1pt
]%
\endinput
% Local variables:
% TeX-master: "../main"
% End:


==> proofs.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{header}
% \myexternaldocument{main}

\begin{document}
\input{authorinf}
% \subtitle{Supplementary Material}

% \begin{abstract}
%   We detail in this document the proofs of correctness.
% \end{abstract}

\maketitle

% \appendix
\input{full-proofs}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> proofs/FullSemanticsRules.tex <==
%
\begin{figure}[t]
  \begin{ruleset}
    \myrule{\mUpgrade}{
      \begin{array}{@{}c@{}}%
        ℓ \trans{% \mode ∧
        g, T}
        ℓ'
      \end{array}
    }{%
      \begin{array}{@{}c@{}}%
        \mframe[]{ℓ}{\V}\H :: \mStack
        \ttrans{\mode ∧ g} T
        \mframe[]{ℓ'}{\V}\H :: \mStack
      \end{array}
    }\\[\myrulespace]
    \myrule{\mBranchRule}{%
      \begin{array}{@{}c@{}}
        \NonJuncL \quad
        ℓ = \semloc{\s{\cif~(e)~\cgoto~\_};\;\_, \_} \\
        c = \V(e) \quad
        ℓ \trans{τ ∧ ¬\mode ∧ g_\tt, T_\tt} ℓ_\tt \quad
        ℓ \trans{¬τ ∧ ¬\mode ∧ g_\ff, T_\ff} ℓ_\ff
      \end{array}
    }{%
      \mframe[]{ℓ}\V \H:: \mStack%
      \ttrans{¬\mode ∧ g_c}{T_c}
      \mframe[]{ℓ_c}\V \H:: \mStack
    }\\[\myrulespace]
    \myrule{\mJunctionRule}{%
      \JuncL{ℓ} \quad ℓ \trans{g, T}ℓ'
    }{%
      \mframe[]{ℓ}\V \H:: \mStack%
      \ttrans{¬\mode ∧ g} T%
      \mframe[]{ℓ'}\V \H:: \mStack%
    }\\[\myrulespace]
    \myrule{\mStmRule}{%
      \begin{array}{@{}c@{}}
        \NonJuncL \quad
        ℓ = \semloc{\stm;\;\_, \_} %
        \trans{g, T}%
        ℓ' \\
        \stm ∈ \mathit{Stm}
        \quad
        \V', \H' = \evalStm\stm(\V, \H)
      \end{array}
    }{%
      \mframe[]{ℓ}\V \H:: \mStack%
      \ttrans{\neg \mode ∧ g} T%
      \mframe[]{ℓ'}{\V'}{ \H'}:: \mStack%
    }\\[\myrulespace]
    \myrule{\mCallRule}{
      \begin{array}{@{}c@{}}
        % \methFrame = \mframe{ℓ}\V \quad
        \methFrame = \mframe[]{ℓ_m}{\V} \H\quad
        \NonJunc{ℓ_m} \quad
     {   ℓ_m = \semloc{\stm;\;\_, \_} %
        \trans{\tt, \_}%
        \_} \\
        \stm = \s{[\_ =]\,r.m'(\lits)} \quad
        \methFrame[m'] = {\NewFrame[\stm, \V, \H]}
      \end{array}
    }{
      \begin{array}{@{}c@{}}%
        \methFrame :: \mStack
        \ttrans{\neg \mode %∧ \SumGuard\stm'
        }{\emptyset}
        \methFrame[m'] :: \methFrame :: \mStack
      \end{array}
    }\\[\myrulespace]
    \myrule{\mExitule}{%
      \begin{array}{@{}c@{}}
        ℓ_{m'} = (\surd, \_) \quad
        \NonJunc{ℓ_{m'}} \quad
        ℓ_m = \semloc{\stm;\_, \_} \trans {\tt,T} ℓ_m'\\
        \stm = [\_=]r.m(w) \qquad \V_m',\H' = [\evalStm{r = \this}(\V, \H) ] \SQMergei u \\
      {\SQMergei u}_{p \in \mathit{Args}_m \cap \MethRefs m}{\evalStm{w^{-1} (p) = p}(\V, \H)}\\
         	{\SQMergei u}
        \begin{cases}
          \evalStm{x=\pi} (\V, \H)
	%          \V_m[x⟼\V_{m'}(π)] 
			& 	\text{if~} \stm = \s{x = \_.m'(\_)}\\
          (\V, \H) & \text{if~} \stm = \s{\_.m'(\_)}
        \end{cases}
        % \evalStm{\s{x = π}}(\V_m［π⟼\V_{m'}(π)］, \H)
      \end{array}
    }{%
      \begin{array}{@{}c@{}}%
        \mframe[]{ℓ_{m'}}{\V_{m'}}{\H_{m'}} :: \mframe[]{ℓ_m}{\V_m}{\H_m} :: \mStack
        \ttrans{% \neg \mode
        \tt}{T}
        \mframe[]{ℓ_m'}{\V_m'}{\H_m'} :: \mStack%
      \end{array}
    }
  \end{ruleset}
%\inote{I'm misusing the notation in Sink rule badly}
  \par
  \smallskip%
  \raggedright%
  where\vspace*{-.2\baselineskip}%
  \setlength{\abovedisplayskip}{0pt}%
  \setlength{\belowdisplayskip}{0pt}%
  \[
    \mathit{Stm} ≝ \!｛\!%
    \begin{array}{@{}c@{}}
      \s{v = e}, \s{v = r.f_p}, \s{r = s}, \s{r = s.f_r}, \\
      \s{r.f_p = e}, \s{r.f_r = s}, \s{r = \cnew\,\_}, \s{r = \Null}, \\
      \s{\creturn}, \s{\creturn\,x}, \s{\cgoto\,\_}, \s{\coutput l (\_)}
    \end{array}%
    \!｝
  \]
  and\vspace*{-.2\baselineskip}%
  \begin{align*}
    % NB: take care e ≡ (r == s)?
     \evalStm{a}(\V, \H) ≝ \,
    \begin{cases}
 \V[v\to {\V}(e)], \H & a =\s{v=e}\\
  \V[v⟼\RefVarsVal \mHeap (r).f_p], \H & a= \s{v = r.f_p} \\
% \evalStm{\s{r = s}}(\V, \H) ≝\, & \V, \NCopyRef r s \H \\
%    \evalStm{\s{r = s.f_r}}(\V, \H) ≝\, & \V, \NSLoadRef r s {f_r} \H \\
%    \evalStm{\s{r.f_p = e}}(\V, \H) ≝\, & \V, \NSStorePrim {r} {f_p} {e} \H \\
%    \evalStm{\s{r.f_r = s}}(\V, \H) ≝\, & \V, \NSStoreRef {r} {f_r} {s} \H \\
%    \evalStm{\s{r = \New~c}}(\V, \H)
%    ≝\, &  \V, \NSNew r c \H \\
%    \evalStm{\s{r = \Null}}(\V, \H) ≝\, & \V, \NNullRef r \H \\
   \V[π⟼\V(v)], \H & a = \s{\creturn~v}\\
    \V, \MemHeapSem {π= r} \H & a=\s{\creturn~r}\\
    \V, \H & a \in \{{\s{\cgoto~\_}},\\
    &\s{\coutput\_(\_)},\s{\creturn}\} \\
    \V, \MemHeapSem{a}\H & \textnormal{otherwise}
  \end{cases}
  \end{align*}
  \caption{Full semantics.}
  \label{fig::full.semantics}
\end{figure}

%\inote{TBD: Will clean up the presentation}
%
% Local variables:
% TeX-master: "main"
% End:


==> proofs/Preliminaries.tex <==
\section{Basic Concepts}
\subsubsection*{Security Domain}
% \label{sec:security-levels}
% We explain our approach by focusing on a confidentiality policy, and
We follow a type-based approach to formalize security where 
security types are assigned to program variables and objects. We consider a 
classical two-level \emph{security domain} that is defined as a
bounded lattice \(〈\LL, ⊑% , ⊥, ⊤, ⊔, ⊓
〉\), where % \todo{≝ for 2 levels?}
\(\LL ⊇ ｛⊥, ⊤｝\) is the finite set of security levels, \(⊑\) is a
partial order defined over \LL{, and \(⊥\) and \(⊤\) respectively
	denote the least (low) and greatest (high) security levels}.
We will typically define a symbolic variable \plvl x to denote the
security level associated with a program variable \(x\).
We then focus on enforcing a confidentiality policy where
high-sensitive (⊤) information should not influence low-sensitive (⊥)
outputs.

\subsubsection*{Input Programs}
\label{sec:input-programs}
We consider input programs as a set of methods that manipulate primitive data, and references to objects.
To maximize the ready availability of our approach%  and better
% demonstrate its practicality
, we concentrate on a low-level language where % the semantics of
most statements % match that of
correspond to %
a family of \Java bytecodes, in a way similar to
\textsf{Jimple}~\citep{vallee2010soot}.
The \emph{body} 
%\MethBody m 
of a method \(m\)
% signature \MethSignFull m
is a non-empty finite
% \(\surd\)-terminated,
semicolon-separated sequence of statements, built according to \stms
in the following grammar:% \figurename~\ref{fig::java.syntax}.
{\setlength\abovedisplayskip{3pt}\setlength\belowdisplayskip{3pt}%
	\[
	\begin{array}{r@{\ }r@{\ }l}
		\stms &⩴& [\lbl{l}:]~\stm;\stms \sep \surd \\
		\stm &⩴& \red{X} \sep [v = ] r.\meth(\lits) \sep \coutput l (\elts)  \sep \creturn~ [v \sep r]
		\\
	\end{array}
	\]}%
where square brackets denote optional constructs,
\(\surd\) is an empty sequence of statements, and \(\lbl{l}\) is a label that uniquely identifies a statement.
\(r.\meth(\lits)\) is a call to the method \meth of the object
referenced by \(r\), with a mapping \lits that associates a
\emph{value} with each formal parameter of \meth.
Our language additionally features a statement \({\coutput
	l(\elts)}\)
that outputs \elts
% given scalar
%values and objects 
to a channel of % a given
security level \(l ∈ \LL\).
\red{X} shows the syntax for intra-procedural  statements, e.g., branches, method invocation-free assignments etc.
%, that we omit in this paper.

\begin{figure}
	\includegraphics[scale=0.2]{Examples/Heap}
	\caption{An example heap model and its symbolic representation}
	\label{fig::heap-model}
\end{figure}


\subsubsection*{Heap Model}
\label{sec:heap-abstraction}
We follow the approach introduced in \cite{SAS} to specify the heap. The heap model maintains 
\begin{itemize}
	\item a \emph{heap typing environment} that
	associates an upper-bound on the security level of the portion of heap
	that is reachable via any reference \(r ∈ R\). The security level of an object refereed by $r$ is denoted by \hlvl[\hvar]r.
	
	\item \emph{over-approximations} of \emph{heap-related relations} between the  reference
	variables in \(R\) and/or the objects that are reachable thereof; this
	notably enables the representation % of multiple levels
	of may-alias relations between % reference
	variables and/or object fields, for instance.
	
\end{itemize}
Let $R$ be a set of references and \red{$\GeneralH$}  be a heap model.
% from an arbitrary heap domain and \(R' \subseteq R\) be a set of references.
The  \emph{reference graph} over \(R\) induced by \GeneralH is a labeled digraph \(\RefGraph{\GeneralH}{R} ≝ \tuple{\Nodes \GeneralH, \Edges\GeneralH}\) where $\Nodes\GeneralH = R$ is the set of nodes, and the edges \Edges\GeneralH show the heap-related relations between the references, \ie
%the label of each node in \Nodes\GeneralH is the reference name,
\(\Edges\GeneralH =\{ (r,\GenericRelSymb,r') ~|~ \GeneralH \models r \GenericRelSymb r', \{r,r'\} \subseteq R\} \).
 \figurename~\ref{fig::heap-model} shows an example heap structure and its symbolic representation.
The nodes show the reference variables and their types, and the edges represent the heap-related relations among references.
The symbolic representation of this example include variables that belong to one of the three following
categories:
\begin{itemize}[nosep]
	\item \ensuremath{\hlvl[]r } holds the \emph{upper bound} on
	the security levels of any object that is reachable via \(r ∈ R\);
	\item \ensuremath{\aliasRel[] r s } is a \emph{may-alias
		variable} for any given \(｛r, s｝⊆ R\), that holds if \(r\) and
	\(s\) may % ~point~to~the~same~object
	alias each other;
	\item \ensuremath{\fieldAliasXRel[] r s } is a
	\emph{transitive field-alias variable}, which holds whenever any object that is \emph{directly}
	referenced by \(s\) \emph{may} be reachable via a reverence field of
	an object that is (indirectly) reachable via \(r\).
\end{itemize}
\begingroup%
\def\fvar{\hvar}%
%Assume for instance a set of reference variables \(R = \{r, s\}\), and
%that any object pointed to by \(s\) may only involve primitive fields
%(\ie we can always assume \(\fieldAliasXRel s r = \fieldAliasXRel s s
%= \ff\)).
%Then, the set of symbolic variables that we use to define an abstract
%heap \fvar that takes its value in the domain \HeapDeepDom R is
%\(\{\hlvl[\fvar] r, \hlvl[\fvar] s: \LL, \aliasRel[\fvar] r s,
%\fieldAliasXRel[\fvar] r r, \fieldAliasXRel[\fvar] r s: \BB\}\).
%%
%We can define 
%every operation %in \tablename~\ref{tab:symbolic-heaps} 
%using this set of variables, such as the predicate that encodes the initialization of
%a given set of references: \(\HeapInit{\{r\}}{\fvar} = \hlvl[\fvar] r =
%⊥ ∧ ¬\aliasRel[\fvar] r s ∧ ¬\fieldAliasXRel[\fvar] r r ∧
%¬\fieldAliasXRel[\fvar] r s\mbox,%
%\) and the update function that encodes the copy of a reference
%variable: \(\NoHeapEffect{r ← s}{\fvar} =
%[\hlvl[\fvar]r\assign\hlvl[\fvar]s, \aliasRel[\fvar]r s \assign \tt,
%\fieldAliasXRel[\fvar] r r \assign \ff, \fieldAliasXRel[\fvar] r s
%\assign \ff]\). 

The expressive power of summaries depend on the chosen heap-related relations (See~\cite{SAS} for the examples of heap abstractions with different heap-related relations). Leaving this set of relations largely unspecified below allows us to abstract away unnecessary details in our exposition where we focus on binary relations without loss of generality.
%	\subsubsection*{Intra-procedural Security Semantics}
%	\label{sec:symbolic-encoding-security-semantics}
%		 \begin{mathpardesc**}
	%		 \item[\G_m] is an SCFG that \emph{encodes the security semantics} of
	%		   \(m\) via a direct translation of its statements%
	%		   % encoding follows a type-based method, so the underlying model
	%		   % assigns
	%		   % % , in addition
	%		   % % with one Boolean controllable input that represents \(m\)'s guard,
	%		   % % and one
	%		   % % (\cf Sections~\ref{sec:enforcing-intra-proc}
	%		   % % and~\ref{sec:interprocedural})
	%		   % % . The construction of the \(\G_m\) follows
	%		   % a security level to each local and formal argument variable, and
	%		   % makes use of a \emph{suitable symbolic heap abstraction} to keep
	%		   % track of the information flow among referenced objects.
	%		   % The latter abstraction, that we seek to keep as generic as possible
	%		   % in our exposition, is also intended to maintain over-approximations
	%		   % of \emph{heap-related relations}---\ie relations that relate
	%		   % references and objects.
	%		   %
	%		   % The resulting model is \emph{flow-sensitive}, meaning that the
	%		   % security level assigned to any variable or object
	%		   % % change during
	%		   % is not fixed for all statement in the program.
	%		   % the program's execution.
	%		   .
	%		   % Last but not least
	%		   The translation algorithm \emph{re\-uses summaries} computed for
	%		   methods called by \(m\) (\eg \(n\) and \(o\) in
	%		   \figurename~\ref{fig:approach-overview-single-method}) to track the
	%		   impact of method calls on explicit and implicit information flows
	%		   and among heap-related relations.
	%		   %
	%		 \item[φ_m] is an \emph{invariant% predicate
		%			   } that expresses a set of safety control objectives:
	%		   \begin{enumerate*}[(i)]
		%			   \item \emph{security properties} % (\eg confidentiality
		%			     % and/or integrity)
		%			     attached to statements%  and method
		%			     % calls% (\cf Section~\ref{sec:enforcing-intra-proc})
		%			     . In the case of confidentiality analysis, such properties
		%			     basically state that no high information may be output on a low
		%			     channel;
		%			   \item an \emph{upper bound constraint} between some
		%			     \emph{controllable variable} π and the security level of the
		%			     returned value, if any, for every sink in the control-flow graph
		%			     of \(m\)—\ie return statements.
		%			     In terms of the model, the above controllable variable is input
		%			     and recorded into a memory variable \(π_X\) in the
		%			     \emph{preamble}, which corresponds to the unique initial
		%			     transition of the induced state machine.
		%			     This means that the strategy to be synthesized via SDCS
		%			     corresponds to a choice of value for π that satisfies the above
		%			     constraint \emph{upon termination} of \(m\), based on security
		%			     levels of arguments and heap-related properties \emph{upon method
			%				       call};
		%			   \item we use a similar mechanism to obtain the security levels of
		%			     objects that \(m\) may mutate (\ie in \Java, every mutable object
		%			     that is reachable via a formal reference argument),
		%			     % security levels as well as on the symbolic heap abstraction
		%			     % induced by formal reference
		%			     % arguments, % , reference relations, etc,
		%			     as well as its effects on relevant heap-related relations.
		%			   \end{enumerate*}
	%		 \item[\K_m] is a synthesized \emph{controller} that ensures:
	%		   \begin{enumerate*}[(i)]
		%			   \item the security properties encoded in \(φ_m\);
		%			   \item a choice for the security level of any returned value, and for
		%			     the security levels and heap-related relations, that satisfies
		%			     every upper bound constraint in \(φ_m\).
		%			     % The latter constraints refer to security levels and relations at
		%			     % every method sink, therefore every choice made by the controller
		%			     % \(\K_m\) \wrt these values satisfy the constraints \emph{upon
			%				     %   method termination}.
		%			     %   Furthermore, t
		%			     This choice is always correct, and the best possible \wrt
		%			     abstractions, due to some property of controllers computed by
		%			     means of SDCS called \emph{maximal permissivity} (\cf
		%			     Section~\ref{sec:princ-discr-contr})%
		%			     % , and this also allows to use \(\K_m\) as a symbolic
		%			     % representation of \(m\)'s effects on its arguments
		%			     .
		%			   \end{enumerate*}
	%		 \item[\MethSum m] is the \emph{symbolic summary}, which results from a
	%		   \emph{triangularization}~\citep{Hietter-triang} of \(\K_m\).
	%		   \MethSum m can be seen as a \emph{function} that outputs:
	%		   \begin{enumerate*}[(i)]
		%			   \item one \emph{guard} for \(m\) that ensures the \emph{security
			%				       properties} based on the security levels of, and relations
		%			     between, its formal arguments;
		%			   % \item one \emph{guard} for each checkpoint statement in \(m\)'s
		%			   %   body;
		%			   \item one \emph{symbolic expression} that expresses the security
		%			     level of \(m\)'s returned value, if any;
		%			   \item one additional \emph{symbolic expression} that describes the
		%			     \emph{potential effect} of \(m\) on the security level of the
		%			     objects it may mutate, as well as on heap-related relations.
		%			     % value as well as returned value, arguments security levels,
		%			     % reference relations, etc, that describes the \emph{potential
			%				     %   effects} of \(m\).
		%			   \end{enumerate*}
	%		 \end{mathpardesc**}
%	 % \begin{redenv}
	%		 % We depict our approach for computing the symbolic summary of a method
	%		 % \(m\) in \figurename~\ref{fig:approach-overview-single-method}:
	%		 % \begin{mathpardesc*}
		%			 % \item[\G_m] is an SCFG that \emph{encodes the security semantics} of
		%			 %   \(m\) via a direct translation of its statements%
		%			 %   % encoding follows a type-based method, so the underlying model
		%			 %   % assigns
		%			 %   % % , in addition
		%			 %   % % with one Boolean controllable input that represents \(m\)'s guard,
		%			 %   % % and one
		%			 %   % % (\cf Sections~\ref{sec:enforcing-intra-proc}
		%			 %   % % and~\ref{sec:interprocedural})
		%			 %   % % . The construction of the \(\G_m\) follows
		%			 %   % a security level to each local and formal argument variable, and
		%			 %   % makes use of a \emph{suitable symbolic heap abstraction} to keep
		%			 %   % track of the information flow among referenced objects.
		%			 %   % The latter abstraction, that we seek to keep as generic as possible
		%			 %   % in our exposition, is also intended to maintain over-approximations
		%			 %   % of \emph{heap-related relations}---\ie relations that relate
		%			 %   % references and objects.
		%			 %   %
		%			 %   % The resulting model is \emph{flow-sensitive}, meaning that the
		%			 %   % security level assigned to any variable or object
		%			 %   % % change during
		%			 %   % is not fixed for all statement in the program.
		%			 %   % the program's execution.
		%			 %   .
		%			 %   % Last but not least
		%			 %   The translation algorithm \emph{re\-uses summaries} computed for
		%			 %   methods called by \(m\) (\eg \(n\) and \(o\) in
		%			 %   \figurename~\ref{fig:approach-overview-single-method}) to track the
		%			 %   impact of method calls on explicit and implicit information flows
		%			 %   and among heap-related relations.
		%			 %   %
		%			 % \item[φ_m] is an \emph{invariant% predicate
			%				 %   } that expresses a set of safety control objectives:
		%			 %   \begin{enumerate*}[(i)]
			%				 %   \item \emph{security properties} % (\eg confidentiality
			%				 %     % and/or integrity)
			%				 %     attached to statements%  and method
			%				 %     % calls% (\cf Section~\ref{sec:enforcing-intra-proc})
			%				 %     . In the case of confidentiality analysis, such properties
			%				 %     basically state that no high information may be output on a low
			%				 %     channel;
			%				 %   \item an \emph{upper bound constraint} between some
			%				 %     \emph{controllable variable} π and the security level of the
			%				 %     returned value, if any, for every sink in the control-flow graph
			%				 %     of \(m\)—\ie return statements.
			%				 %     In terms of the model, the above controllable variable is input
			%				 %     and recorded into a memory variable \(π_X\) in the
			%				 %     \emph{preamble}, which corresponds to the unique initial
			%				 %     transition of the induced state machine.
			%				 %     This means that the strategy to be synthesized via SDCS
			%				 %     corresponds to a choice of value for π that satisfies the above
			%				 %     constraint \emph{upon termination} of \(m\), based on security
			%				 %     levels of arguments and heap-related properties \emph{upon method
				%					 %       call};
			%				 %   \item we use a similar mechanism to obtain the security levels of
			%				 %     objects that \(m\) may mutate (\ie in \Java, every mutable object
			%				 %     that is reachable via a formal reference argument),
			%				 %     % security levels as well as on the symbolic heap abstraction
			%				 %     % induced by formal reference
			%				 %     % arguments, % , reference relations, etc,
			%				 %     as well as its effects on relevant heap-related relations.
			%				 %   \end{enumerate*}
		%			 % \item[\K_m] is a synthesized \emph{controller} that ensures:
		%			 %   \begin{enumerate*}[(i)]
			%				 %   \item the security properties encoded in \(φ_m\);
			%				 %   \item a choice for the security level of any returned value, and for
			%				 %     the security levels and heap-related relations, that satisfies
			%				 %     every upper bound constraint in \(φ_m\).
			%				 %     % The latter constraints refer to security levels and relations at
			%				 %     % every method sink, therefore every choice made by the controller
			%				 %     % \(\K_m\) \wrt these values satisfy the constraints \emph{upon
				%					 %     %   method termination}.
			%				 %     %   Furthermore, t
			%				 %     This choice is always correct, and the best possible \wrt
			%				 %     abstractions, due to some property of controllers computed by
			%				 %     means of SDCS called \emph{maximal permissivity} (\cf
			%				 %     Section~\ref{sec:princ-discr-contr})%
			%				 %     % , and this also allows to use \(\K_m\) as a symbolic
			%				 %     % representation of \(m\)'s effects on its arguments
			%				 %     .
			%				 %   \end{enumerate*}
		%			 % \item[\MethSum m] is the \emph{symbolic summary}, which results from a
		%			 %   \emph{triangularization}~\citep{Hietter-triang} of \(\K_m\).
		%			 %   \MethSum m can be seen as a \emph{function} that outputs:
		%			 %   \begin{enumerate*}[(i)]
			%				 %   \item one \emph{guard} for \(m\) that ensures the \emph{security
				%					 %       properties} based on the security levels of, and relations
			%				 %     between, its formal arguments;
			%				 %   % \item one \emph{guard} for each checkpoint statement in \(m\)'s
			%				 %   %   body;
			%				 %   \item one \emph{symbolic expression} that expresses the security
			%				 %     level of \(m\)'s returned value, if any;
			%				 %   \item one additional \emph{symbolic expression} that describes the
			%				 %     \emph{potential effect} of \(m\) on the security level of the
			%				 %     objects it may mutate, as well as on heap-related relations.
			%				 %     % value as well as returned value, arguments security levels,
			%				 %     % reference relations, etc, that describes the \emph{potential
				%					 %     %   effects} of \(m\).
			%				 %   \end{enumerate*}
		%			 % \end{mathpardesc*}
	%		 % \end{redenv}
%	 We focus on specific modeling concerns in each subsection, and
%	 therefore construct the sets \(X_m\), \(U_m\), and \(C_m\)
%	 incrementally% way in accord with
%	 % Remark~\ref{rem:incremental-definition-of-update-functions}
%	 .
%	 \label{sec:notion:heap-objects}
%	 Using the above notations, one can now define the set of all
%	 allocation sites as \(\HH ≝ ⋃_{m∈��}｛h∈\pp m｜h = ⟪r = \cnew~c⟫｝\).
%	 We
%	 %will % first consider the case of a single method body without method
%	 % calls% , that will give us the basis for the definition and computation
%	 % % of summaries
%	 % , and
%	 elaborate on the definition, computation, and re-use of symbolic
%	 summaries % in order
%	 to deal with method
%	 calls% to handle full programs \red{(call-graphs)}
%	 We also introduce operations required for the symbolic heap
%	 abstraction in parallel;
%	 % \red{, and terminate this Section with more details on such aspects
	%		 % along with an example}.
%	 %
%	 for ease of reference% , however
%	 , we list them in
%	 \tablename~\ref{tab:symbolic-heaps}% all operations required on
%	 % symbolic heap abstractions
%	 , associated with the domain of the resulting expressions.
%	
%	We illustrate the application of translation rules with the example
%	SCFG given in \figurename~\ref{fig:c-bar-example-scfg}.
%	This SCFG results from the translation of the sequence of statements
%	given in \figurename~\ref{fig:c-bar-cdrs-illustration}, which is
%	itself derived from our example code of
%	\lstlistingname~\ref{lst:c-bar-example-code}.
%	This SCFG additionally comprises several parts that we use to
%	illustrate the computation and re\-use of summaries in
%	Section~\ref{sec:interprocedural}, namely a preamble transition, a
%	desired invariant on the sink location, and a location that
%	corresponds to a method call.
%	
%	We % follow a type-based approach, and
%	first define a \emph{security typing environment} for each primitive
%	or reference variable in \MethBody m.
%	This environment is
%	% and a heap abstraction
%	symbolically encoded by means of state variables (\ie they belong to
%	the set \(X_m\) of the SCFG) as
%	% Generated SCFGs involve several state variables that constitute a
%	% symbolic encoding of a % encode the
%	% security semantics of the program in terms of explicit or indirect
%	% information flows, %
%	% (belonging to the vector \(X\)) (we introduce additional state
%	% variables in Section~\ref{notion:capt-indir-inform} to account for
%	% indirect information flows)
%	%


